Assessment of a cost-effective headphone calibration procedure for soundscape evaluations

To increase the availability and adoption of the soundscape standard, a low-cost calibration procedure for reproduction of audio stimuli over headphones was proposed as part of the global ``Soundscape Attributes Translation Project'' (SATP) for validating ISO/TS~12913-2:2018 perceived affective quality (PAQ) attribute translations. A previous preliminary study revealed significant deviations from the intended equivalent continuous A-weighted sound pressure levels ($L_{\text{A,eq}}$) using the open-circuit voltage (OCV) calibration procedure. For a more holistic human-centric perspective, the OCV method is further investigated here in terms of psychoacoustic parameters, including relevant exceedance levels to account for temporal effects on the same 27 stimuli from the SATP. Moreover, a within-subjects experiment with 36 participants was conducted to examine the effects of OCV calibration on the PAQ attributes in ISO/TS~12913-2:2018. Bland-Altman analysis of the objective indicators revealed large biases in the OCV method across all weighted sound level and loudness indicators; and roughness indicators at \SI{5}{\%} and \SI{10}{\%} exceedance levels. Significant perceptual differences due to the OCV method were observed in about \SI{20}{\%} of the stimuli, which did not correspond clearly with the biased acoustic indicators. A cautioned interpretation of the objective and perceptual differences due to small and unpaired samples nevertheless provide grounds for further investigation.

==> [ICA22] Calibration/table/cfstats.tex <==
\begin{table}[t]
\caption{Accuracy, sensitivity, specificity, and precision, and McNemar's Test \textit{p}-value of the WHO and WHO+ grading criteria for normal hearing. WHO+ includes the measurements at 6 kHz in the grading, which is on top of the 4 frequencies in the WHO grading (i.e. 0.5, 1, 2, and \SI{4}{\kilo\hertz}).}
\centering
\begin{tabularx}{\textwidth}{lc*{3}{>{\centering\arraybackslash}X}c}
\toprule
Grading                     &   
Accuracy (\%; \SI{95}{\%} CI)  &   
Sensitivity (\%)            &   
Specificity (\%)            &   
Precision (\%)              &
MNT \textit{p}-value            \\

\midrule
WHO                     &   
95.09 (90.56, 97.86)        &   
96.77                       &   
62.50                       &   
98.04                       &
0.723                       \\

WHO+                           &   
98.16 (94.72, 99.62)        &   
99.34                       &   
81.82                       &   
98.69                       &
1.000                        \\
\bottomrule
\end{tabularx}
\label{tab:cfmetrics}
\end{table}

==> [ICA22] Calibration/table/malay_translations.tex <==
\begin{table}[t]
    \centering
    \caption{ISO/TS 12913-2 PAQ attributes and corresponding candidate translations in Malay used for the subjective assessment of the OCV and HATS calibrations methods in this study.} % Add \usepackage{caption} to allow line breaks in long captions.
    \begin{tabular}{cc}
        \toprule
        ISO/TS 12913-2 PAQ attribute & Candidate translation in Malay \\
        \midrule
        pleasant & menyenangkan \\
        chaotic & huru-hara \\
        vibrant & rancak \\
        uneventful & tidak meriah \\
        calm & tenang \\
        annoying & membingitkan \\
        eventful & meriah \\
        monotonous & membosankan \\
        \bottomrule
    \end{tabular}
    \label{tab:malay_translations}
\end{table}


==> [ICA22] Calibration/table/wrs.tex <==
\begin{table}[t]
\centering
\caption{Wilcoxon signed rank tests, and the pseudomedian and its confidence intervals (\SI{}{\decibel} HL; 95\% confidence level) of the differences between the audiometer and uHear audiograms are computed at each frequency (0.5, 1, 2, 4 and \SI{6}{\kilo\hertz}) across both ears. The null hypothesis is rejected at \textit{p}-value $<0.05$.}
\setlength{\tabcolsep}{12pt}
\begin{tabularx}{\textwidth}{%
    X
    S[table-format=1.1]
    S[table-format=-1.1]
    r@{\hskip0pt}S[table-format=-1.1,table-space-text-pre={[}]
    @{,\hskip-35pt}S[table-format=-1.1]<{{)}}
    S[table-format=1.2e2]}
\toprule
Ear & {Frequency (\si{\kilo\hertz})} & {Pseudomedian} & \multicolumn{3}{c}{Confidence Interval (\SI{95}{\%})\qquad}  & \multicolumn{1}{c}{\textit{p}-value}\\
\midrule
\multirow{5}{*}{\centering\arraybackslash Left}
& 0.5 & -5.0 &\qquad(&-5 & -5& 6.11e-7\\

& 1 & -7.5  &\qquad(&-7.5 & -7.5& 3.37e-19\\

& 2 & -5.0  &\qquad(&-7.5 & -2.5& 7.14e-7\\

& 4 & -5.0  &\qquad(&-7.5 & -5& 1.65e-10\\

& 6 & 2.5  &\qquad(&0 & 5& 1.13e-3\\
    
\midrule
\multirow{5}{*}{\centering\arraybackslash Right}
& 0.5 & -5.0  &\qquad(&-5 & -2.5& 2.14e-6\\

& 1 & -7.5  &\qquad(&-7.5 & -7.5& 4.31e-23\\

& 2 & -5.0  &\qquad(&-7.5 & -5& 1.61e-13\\

& 4 & -7.5  &\qquad(&-7.5 & -7.5& 1.67e-16\\

& 6 & 2.5  &\qquad(&0 & 2.5& 6.82e-2\\
\bottomrule
\end{tabularx}
\label{tab:wrs_results}
\end{table}



==> table/cfstats.tex <==
\begin{table}[t]
\caption{Accuracy, sensitivity, specificity, and precision, and McNemar's Test \textit{p}-value of the WHO and WHO+ grading criteria for normal hearing. WHO+ includes the measurements at 6 kHz in the grading, which is on top of the 4 frequencies in the WHO grading (i.e. 0.5, 1, 2, and \SI{4}{\kilo\hertz}).}
\centering
\begin{tabularx}{\textwidth}{lc*{3}{>{\centering\arraybackslash}X}c}
\toprule
Grading                     &   
Accuracy (\%; \SI{95}{\%} CI)  &   
Sensitivity (\%)            &   
Specificity (\%)            &   
Precision (\%)              &
MNT \textit{p}-value            \\

\midrule
WHO                     &   
95.09 (90.56, 97.86)        &   
96.77                       &   
62.50                       &   
98.04                       &
0.723                       \\

WHO+                           &   
98.16 (94.72, 99.62)        &   
99.34                       &   
81.82                       &   
98.69                       &
1.000                        \\
\bottomrule
\end{tabularx}
\label{tab:cfmetrics}
\end{table}

==> table/malay_translations.tex <==
\begin{table}[t]
    \centering
    \caption{ISO/TS 12913-2 PAQ attributes and corresponding candidate translations in Malay used for the subjective assessment of the OCV and HATS calibrations methods in this study.} % Add \usepackage{caption} to allow line breaks in long captions.
    \begin{tabular}{cc}
        \toprule
        ISO/TS 12913-2 PAQ attribute & Candidate translation in Malay \\
        \midrule
        pleasant & menyenangkan \\
        chaotic & huru-hara \\
        vibrant & rancak \\
        uneventful & tidak meriah \\
        calm & tenang \\
        annoying & membingitkan \\
        eventful & meriah \\
        monotonous & membosankan \\
        \bottomrule
    \end{tabular}
    \label{tab:malay_translations}
\end{table}


==> table/wrs.tex <==
\begin{table}[t]
\centering
\caption{Wilcoxon signed rank tests, and the pseudomedian and its confidence intervals (\SI{}{\decibel} HL; 95\% confidence level) of the differences between the audiometer and uHear audiograms are computed at each frequency (0.5, 1, 2, 4 and \SI{6}{\kilo\hertz}) across both ears. The null hypothesis is rejected at \textit{p}-value $<0.05$.}
\setlength{\tabcolsep}{12pt}
\begin{tabularx}{\textwidth}{%
    X
    S[table-format=1.1]
    S[table-format=-1.1]
    r@{\hskip0pt}S[table-format=-1.1,table-space-text-pre={[}]
    @{,\hskip-35pt}S[table-format=-1.1]<{{)}}
    S[table-format=1.2e2]}
\toprule
Ear & {Frequency (\si{\kilo\hertz})} & {Pseudomedian} & \multicolumn{3}{c}{Confidence Interval (\SI{95}{\%})\qquad}  & \multicolumn{1}{c}{\textit{p}-value}\\
\midrule
\multirow{5}{*}{\centering\arraybackslash Left}
& 0.5 & -5.0 &\qquad(&-5 & -5& 6.11e-7\\

& 1 & -7.5  &\qquad(&-7.5 & -7.5& 3.37e-19\\

& 2 & -5.0  &\qquad(&-7.5 & -2.5& 7.14e-7\\

& 4 & -5.0  &\qquad(&-7.5 & -5& 1.65e-10\\

& 6 & 2.5  &\qquad(&0 & 5& 1.13e-3\\
    
\midrule
\multirow{5}{*}{\centering\arraybackslash Right}
& 0.5 & -5.0  &\qquad(&-5 & -2.5& 2.14e-6\\

& 1 & -7.5  &\qquad(&-7.5 & -7.5& 4.31e-23\\

& 2 & -5.0  &\qquad(&-7.5 & -5& 1.61e-13\\

& 4 & -7.5  &\qquad(&-7.5 & -7.5& 1.67e-16\\

& 6 & 2.5  &\qquad(&0 & 2.5& 6.82e-2\\
\bottomrule
\end{tabularx}
\label{tab:wrs_results}
\end{table}


